Abstraction Logic: The Marriage of Contextual Refinement and Separation Logic

Contextual refinement and separation logics are successful verification techniques that are very different in nature. First, the former guarantees behavioral refinement between a concrete program and an abstract program while the latter guarantees safety of a concrete program under certain conditions (expressed in terms of pre and post conditions). Second, the former does not allow any assumption about the context when locally reasoning about a module while the latter allows rich assumptions. In this paper, we present a new verification technique, called abstraction logic (AL), that inherently combines contextual refinement and separation logics such as Iris and VST, thereby taking the advantages of both. Specifically, AL allows us to locally verify a concrete module against an abstract module under separation-logic-style pre and post conditions about external modules. AL are fully formalized in Coq and provides a proof mode that supports a combination of simulation-style reasoning using our own tactics and SL-style reasoning using IPM (Iris Proof Mode). Using the proof mode, we verified various examples to demonstrate reasoning about ownership (based on partial commutative monoids) and purity ($i.e.$, termination with no system call), cyclic and higher-order reasoning about mutual recursion and function pointers, and reusable and gradual verification via intermediate abstractions. Also, the verification results are combined with CompCert, so that we formally establish behavioral refinement from top-level abstract programs, all the way down to their assembly code.

==> evaluation.tex <==
\section{Evaluation and Discussion}
\label{sec:evaluation}

\begin{wrapfigure}{R}{5.0cm}
\begin{minipage}{\linewidth}
\vspace{-5mm}
\parbox{0.33\linewidth}{
\begin{tabu}{l @{\;}|@{\;} l @{\;}|@{\;} l}
Portion & Spec & Proof \\
\hline
Examples & 2099 & 1436 \\ %% examples + mem.
Meta-Theories & 6808 & 5376 \\ %% theories + open(currently in mem directory)
Imp & 3150 & 3799 \\ %% imp
Libraries & 3029 & 862 \\ %% extraction && libraries
\hline
Total & 17859 & 14041 \\
\end{tabu}
\label{table:evaluation-breakdown}
}
\end{minipage}
\vspace{-3mm}
\end{wrapfigure}

The right table analyzes our whole development in terms of SLOC (measured with
\code{coqwc}). First, SLOC of our examples (Cannon, Mem, Stack, Echo, \yj{Repeat}, Mutual
sum, Landin's knot) amounts to 77777. In our experience, verification effort in \crems{} is
comparable to that of Iris (since we use IPM).



\todo{디렉토리 정리. 스크립트 짜기. @dongjaelee}

\yj{say that our meta theory uses gradual verification heavily}

\yj{say that execution is useful. segfault type error}

\yj{LOC is comparable to that of separation logic}


\myparagraph{(\rom{5}) Extraction and Execution} Our examples, embedded in \ems, can be
extracted to OCaml and executed \eg at top level ($\overline{A}$) and \imp level ($I$). Also,
recall that we have a verified compiler from \imp to CompCert Csharpminor, which in turn
allows execution in assembly level ($Asm$). We will share our experience, current limitations, and
possible future works.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> stack.tex <==
\gil{======= Old draft ========}

\section{Stack}
More specifically, we define \ems~(Executable Module Semantics) as an executable semantics\footnote{
  By an executable semantics, we mean an operational semantics that can be extracted to OCaml via Coq's extraction mechanism, allowing to approximate uncomputable expressions into computable ones.
} based on Interaction Trees~\cite{liyao:itree}, into which semantics of various implementation and specification languages can be embedded.
Then, a \emph{closed} \ems semantics gives a set of behaviors (derived from its execution steps) each of which is a finite or infinite sequence of observable events (\eg as in CompCert~\cite{CompCert}).
From this, we can define the notion of contextural refinement between two \emph{open} \ems semantics $S_1, S_2$ in the standard way:
we say $S_1$ \emph{contextually refines} $S_2$, denoted $S_1 \lectx S_2$, if for any context \ems $C$\footnote{Technically speaking, we allow the context to consist of arbitrary number of context modules $C_1,\ldots,C_n$.} such that $C \link S_1$ and $C \link S_2$ are closed for the linking operator $\link$,
the set of behaviors of $C \link S_1$ is a subset of that of $C \link S_2$.
Finally, we say that an implementation or specification is verified against another (typically more abstract) implementation or specification if we establish contextual refinement between their \ems semantics.

\subsection{High-level overview of \crems}
%% To give a high-level overview,
We briefly discuss how \crems looks and works using a motivating example, \code{\kwmodule Echo},
whose implementation \echoimpl given in \Cref{fig:echo-impl-old} is written in a C-like implementation language \imp.
In \echoimpl, \code{Echo.echo()} creates a new stack, \code{stk}, setting the reserved value for checking emptiness to be \code{\exitval};
invokes \code{Echo.input(stk)}, which repeatedly gets an integer via \code{IO.getint} and pushes it into \code{stk} until getting \code{\exitval};
and then invokes \code{Echo.output(stk)}, which repeatedly pops an integer from \code{stk} and outputs it via \code{IO.putint} until the stack is empty
(\ie the reserved value \code{\exitval} is returned).
Note that \imp uses dynamically typed values consisting of integers and pointers including function pointers as in C.
Also, in \Cref{?}, we will discuss how to embed \imp (more generally, any dynamically or statically typed languages) into \ems,
where they need to interact with arbitrary \ems contexts that may provide \emph{arbitrary mathematical values}.

We first discuss limitations of contextual refinement and separation logics for \code{\kwmodule Echo}.
In the former, since one cannot make any assumption about the external modules,
there is only a tiny room for giving a more abstract specification such as reducing the number of exit points in \code{output} as follows:
\[
   \code{... if (v != \exitval) \{ IO.putint(v); output(stk) \}; () }
\]
On the other hand, in the latter, one can choose specifications (\ie specific pre and post conditions) for all modules including \code{Echo}, \code{Stack}, \code{IO}
and separately verify each module against its own specification assuming the chosen specifications for the other modules, which then collectively guarantees safety of the whole system.
A limitation here is that one has to verify safety of \emph{all} modules including even \code{IO}, which may not be a good target for verification or even giving a specification, for example, because it might be unknown code (possibly making recursive calls to \code{Echo}) or depend on user's unpredictable behavior.
A more desirable specification would be to directly specify possible interactions with an arbitrary (unverified) \code{IO} module.

\begin{figure}[t]
\begin{minipage}{0.34\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Echo]
\kwdef echo() $\equiv$
  \kwvar stk := Stack.new(\exitval);
  Echo.input(stk);
  Echo.output(stk)
\end{Verbatim}
\end{minipage}%
\begin{minipage}{0.35\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef input(stk) $\equiv$
  \kwvar v := IO.getint();
  \kwif (v == \exitval) ()
  \kwelse \{ Stack.push(stk, v);
         Echo.input(stk) \}
\end{Verbatim}
\end{minipage}%
\begin{minipage}{0.31\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef output(stk) $\equiv$
  \kwvar v := Stack.pop(stk);
  \kwif (v == \exitval) ()
  \kwelse \{ IO.putint(v);
         Echo.output(stk) \}
\end{Verbatim}
\end{minipage}
\caption{\echoimpl: An implementation of \code{\kwmodule Echo} in \imp}
\label{fig:echo-impl-old}
\end{figure}

\begin{figure}[t]
\begin{minipage}{0.55\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
[\kwmodule Echo]
// pre \& post conditions
\kwspec Stack.new: ...
\kwspec Stack.push: ...
\kwspec Stack.pop: ...
\kwspec Echo.input: ...
\kwspec Echo.output: ...
\kwspec Echo.echo: \kwdefault
\kwspec IO.getint: \kwdefault
\kwspec IO.putint: \kwdefault

\kwdef echo \{
  \kwcontext,\kwfriend () $\equiv$
    \kwvar stk: list int := Echo.input([]);
    Echo.output(stk)
\}  
\end{Verbatim}
\end{minipage}%
\hfill%
\begin{minipage}{0.45\textwidth}
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3},fontsize=\small]
\kwdef input \{
  \kwcontext (stk) $\equiv$ \kwassume{(false)}
  \kwfriend (stk: list int): list int $\equiv$
    \kwvar v: int := $\downcast{\code{IO.getint()}}$;
    \kwif (v == \exitval) stk
    \kwelse Echo.input(v :: stk)
\}  
\kwdef output \{
  \kwcontext (stk) $\equiv$ \kwassume{(false)}
  \kwfriend (stk: list int): unit $\equiv$
    \kwmatch stk \kwwith
    | [] => ()
    | v :: stk' => IO.putint($\upcast{\code{v}}$);
                   Echo.output(stk')
    \kwend
\}                 
\end{Verbatim}
\end{minipage}%
\caption{\echospec: A specification of \code{\kwmodule Echo} in \spc}
\label{fig:echo-spec}
\end{figure}

%% Now we will highlight how \crems is different from the others by briefly discussing how the \code{Echo} module is verified in \crems.

In \crems, one can indeed write such a desirable specification, \echospec shown in \Cref{fig:echo-spec}, which is written in a specification language, called \spc
(Separation Logic with GENeral computation).
The first part (starting with \kwspec, which is hidden for a presentation purpose and will be shown in \Cref{???}) includes specific pre and post conditions for \code{Echo} and \code{Stack}
(similar to what one would write in a separation logic like \iris)
but not for \code{IO} because we intend to leave \code{IO} as a part of \emph{completely unrestricted} contexts 
(\ie arbitrary {\ems}es, which may be unsafe or make arbitrary calls including recursive calls to \code{Echo} and \code{Stack}).
%% The second part includes \emph{executable} specifications of \code{Echo} for
The second part (starting with \kwfriend, ignoring \kwcontext for now) presents a more direct and abstract version of \code{Echo}'s computation, which uses the mathematical \code{list int} datatype instead of relying on the \code{Stack} module.
Specifically, \code{Echo.echo()} invokes \code{Echo.input} with the empty list \code{[]},
which repeatedly accumulates an integer received via \code{IO.getint} in the list and returns it when receiving \code{\exitval};
%% repeatedly gets an integer via \code{IO.getint} and accumulate it in the list until getting \code{\exitval}, and finally returns the accumulated list;
and then invokes \code{Echo.output} with the returned list \code{stk},
which repeatedly pops the head of the list and outputs it via \code{IO.putint}.
% until the stack is empty.

Now, we look into how this example works in \crems at a high-level.

  In \spc, one can use any mathematical datatypes (\ie sets) and their values, and the input and output types of each function is specified in its pre and post conditions.
  For example, since \code{IO.getint} has no specification, its return type is \code{Any}, which, roughly speaking, is the set of all mathematical values,
  and thus we \emph{downcast} the return value of \code{IO.getint()} into an integer using the operator $\downcast{}$ (colored in red).
  Note that we color operators in red when its failure triggers the usual notion of \emph{undefined behavior (UB)}, which is interpreted as all possible behaviors.
  Conversely, we \emph{upcast} an integer to \code{Any} using $\upcast{}$ when passing it to \code{IO.putint}.

  Every specification written in \spc also gives an executable semantics in \ems,
  which involves two (\ie usual and unusual) kinds of nondeterminism in order to $(i)$ turn the pre and post conditions involving PCMs into an operational semantics, and $(ii)$ merge the two definitions with \kwcontext and \kwfriend into a single definition.
  Note, however, that such nondeterminism will be automatically eliminated later.

  For verification of the \code{Echo} module, we prove contextual refinement between the \ems semantics of \echoimpl and that of \echospec.
  By using the \crems proof mode in Coq, we greatly streamline the proof, which is essentially similar to what one would write for similar pre and post conditions in a separation logic like \iris.
  An interesting point here is that the proof establishes behavioral refinement under arbitrary contexts even including \code{Stack},
  which may sound contradictory, \eg because \code{Stack.new}, an arbitrary function that may even crash, is invoked in \echoimpl but not in \echospec.
  However, this is not a contradiction because, at any point during execution, \spc implicitly and non-deterministically invokes arbitrary functions that are specified as \emph{pure}\footnote{%
    \crems provides a way to specify purity (\ie not producing any side effects such as non-termination, fatal errors, or system calls).
  } in their pre and post conditions, which is the case for \code{Stack.new}, \code{Stack.push} and \code{Stack.pop} in \echospec.
  Also note that all such invocations of pure functions will be automatically eliminated later.

  \crems provides \emph{\checker}. Given $S_1,\ldots,S_n$ written in \spc, called \emph{friends},
  it $(i)$ checks compatibility between the pre and post conditions written in the friends, which in particular requires \kwspec of \emph{context modules} (\ie non-friends) appearing in $S_i$ such as \code{IO} to be \kwdefault;
  $(ii)$ produces corresponding modules $G_1,\ldots,G_n$ written in \gen (a language for describing general computation) by eliminating the logical specification parts (starting with \kwspec) from $S_1,\ldots, S_n$;
  and $(iii)$ establishes contextual refinement between them: $S_1 \link \ldots \link S_n \lectx G_1 \link \ldots \link G_n$.
  Note, in particular, that all unusual nondeterminism and implicit invocations introduced in \spc are eliminated by \checker.
  In the \code{Echo} example, with \checker we turn the specifications \echospec, \stackspec, \memspec of \code{Echo}, \code{Stack} and \code{Mem} (but not \code{IO}) into general computations \echogen, \stackgen, \memgen,
  where \code{Mem} is the memory module for \imp with four functions, \kwmalloc, \kwfree, \kwload, \kwstore, and used by the \code{Stack} module.

  Concretely, the produced modules $G_1,\ldots,G_n$ are simple combinations of the \kwfriend and \kwcontext definitions in $S_1,\ldots,S_n$,
  where a function $f$ in $G_i$, when invoked, $(i)$ checks whether the caller module is a friend (\ie whether the caller module's name is among the module names of $S_1,\ldots,S_n$\footnote{A function call in \ems also passes the module name of the caller to the callee as meta information.});
  $(ii)$ if so, executes the \kwfriend definition of the function $f$ in $S_i$; $(iii)$ otherwise, executes its \kwcontext definition.
  For example, in \echospec, if context modules including \code{IO} invoke \code{Echo.input} or \code{Echo.output},
  their \kwcontext definitions, \code{\kwassume{(false)}}, immediately trigger UB, which captures the intention that context modules are not allowed to call those functions.
  On the other hand, since the \kwcontext definition of \code{Echo.echo} is the same as its \kwfriend definition,
  context modules can successfully invoke it.
  
  With \kwfriend and \kwcontext in minds, we revisit the verification of \code{Echo}.
  Actually, proving $\echoimpl \lectx \echospec$ essentially requires to prove two refinements for each function $f$ in \code{Echo}:
  $(i)$ refinement between $f$ in \echoimpl and the \kwfriend definition of $f$ in \echospec with respect to the pre and post conditions of $f$ in \echospec,\footnote{
    The relationship between argument/return values in the source and target is specified in the pre and post conditions of $f$.
    } and
  $(ii)$ refinement between $f$ in \echoimpl and the \kwcontext definition of $f$ in \echospec with respect to the \kwdefault specification.
  In the \code{Echo} example, the latter refinements for \code{Echo.input} and \code{Echo.output} trivially hold since their \kwcontext definitions immediately trigger UB;
  and for \code{Echo.echo}, its former and latter refinements coincide since the two definitions are the same and their specifications are both \kwdefault.

  Finally, it is also possible to leave assumptions and guarantees about specific properties in the resulting specifications $G_1,\ldots,G_n$.
  For example, for any predicate $P$ on \code{int}, suppose we change \echospec to $\echospec'$ by inserting \code{\kwassume($P$(v))} just after getting \code{v} via \code{IO.getint}
  and \code{\kwguarantee($P$(v))} just before passing \code{v} to \code{IO.putint}.
  Here \code{\kwassume($P$(v))} operationally captures the intuition that we \emph{assume} the input integer \code{v} satisfies $P$,
  while \code{\kwguarantee($P$(v))} that we \emph{guarantee} the output integer \code{v} must satisfy $P$ (see \Cref{?} for the definitions).
  %% Here \code{\kwassume($P$(v))} triggers UB if \code{$P$(v)} does not hold, and does nothing otherwise, which captures that we \emph{assume} the input integer \code{v} satisfies $P$.
  %% On the other hand, \code{\kwguarantee($P$(v))} triggers the dual of UB, called \emph{NB} (No Behavior), if \code{$P$(v)} does not hold, and does nothing otherwise, which captures that we \emph{guarantee} the output integer \code{v} must satisfy $P$.
  Then we can prove $\echoimpl \lectx \echospec'$ with extra reasoning that every value in the list satisfies $P$.
  After using \checker, we get $\echogen'$, which will still contain \code{\kwassume($P$(v))} and \code{\kwguarantee($P$(v))}.
  % which operationally state the intended assumption and guarantee.
  
  To sum up, a general scenario in \crems is as follows.
  Given implementations $I_1,\ldots,I_n$ (in \imp or any other language), we can write intended specifications $S_1,\ldots,S_n$ in \spc and separately prove $I_i \lectx S_i$ for each module.
  Then we can use \checker to produce $G_1, \ldots, G_n$ with $S_1 \link \ldots \link S_n \lectx G_1 \link \ldots \link G_n$.
  By composing the contextual refinements horizontally and vertically, we get $I_1 \link \ldots \link I_n \lectx G_1 \link \ldots \link G_n$, which guarantees behavioral refinement under arbitrary context modules.
  Furthermore, since $G_1, \ldots, G_n$ can be seen as implementations written in \gen, one can further verify them (possibly together with other implementations for extra modules) against more abstract specifications.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

